An Event Based Approach To Situational Representation

Many application domains require representing interrelated real-world activities and/or evolving physical phenomena. In the crisis response domain, for instance, one may be interested in representing the state of the unfolding crisis (e.g., forest fire), the progress of the response activities such as evacuation and traffic control, and the state of the crisis site(s). Such a situation representation can then be used to support a multitude of applications including situation monitoring, analysis, and planning. In this paper, we make a case for an event based representation of situations where events are defined to be domain-specific significant occurrences in space and time. We argue that events offer a unifying and powerful abstraction to building situational awareness applications. We identify challenges in building an Event Management System (EMS) for which traditional data and knowledge management systems prove to be limited and suggest possible directions and technologies to address the challenges.

==> challenges.tex <==
\subsection{Challenges}
\label{sec:challenges}

In this section, we discuss challenges we plan to address in near future for making EDBMS a reality.

\begin{itemize}

\item
{\em Ontology-driven event extraction.} To populate the EventWeb it is necessary to {\em extract} information from the raw datasets and instantiate the according ontologies. This problem is known to be difficult if the ontology is not fixed, however it is considered manageable for fixed ontologies. 

\item
{\em Disambiguation.} After the information is extracted from raw data, it is frequently inherently uncertain. For example, it might be hard to determine if the two extracted events are the same or not, based on the provided descriptions of the events. To be able to initialize the EventWeb it is necessary to be able to handle uncertainty in data. We have succeeded at solving of only two disambiguation problems, known as ``reference disambiguation" and ``object consolidation", as summarized in Section~\ref{sec:disamb}. However, other disambiguation challenges are yet to be addressed.

\item
{\em Handling uncertainty in data.} The challenge is to design solutions that are capable of handling the inherent uncertainty in data. For example, people tend to specify locations in an imprecise manner, in terms of the relationships that exists between the locations and nearby landmarks. The information about the precise point-location of the event might not be stored anywhere in the database. Nevertheless, the system should provide support for analytical queries on top of such uncertain information, for spatial and other types of data. We discuss one approach to deal with uncertain event location in Section~\ref{sec:uncloc}.

\item
{\em Analysis tools.} The decision makers should be provided with tools/API to interface with Event DBMS to enable reasoning about stored events. Creating such a functionality requires solving several research and technical challenges.
\end{itemize} 

